May the Force be with You: Unified Force-Centric Pre-Training for 3D Molecular Conformations

Recent works have shown the promise of learning pre-trained models for 3D molecular representation. However, existing pre-training models focus predominantly on equilibrium data and largely overlook off-equilibrium conformations. It is challenging to extend these methods to off-equilibrium data because their training objective relies on assumptions of conformations being the local energy minima. We address this gap by proposing a force-centric pretraining model for 3D molecular conformations covering both equilibrium and off-equilibrium data. For off-equilibrium data, our model learns directly from their atomic forces. For equilibrium data, we introduce zero-force regularization and forced-based denoising techniques to approximate near-equilibrium forces. We obtain a unified pre-trained model for 3D molecular representation with over 15 million diverse conformations. Experiments show that, with our pre-training objective, we increase forces accuracy by around 3 times compared to the un-pre-trained Equivariant Transformer model. By incorporating regularizations on equilibrium data, we solved the problem of unstable MD simulations in vanilla Equivariant Transformers, achieving state-of-the-art simulation performance with 2.45 times faster inference time than NequIP. As a powerful molecular encoder, our pre-trained model achieves on-par performance with state-of-the-art property prediction tasks.

==> exp/backup.tex <==

\paragraph{The pretraining stage is essential for }

\begin{table}[h]
    \centering
    \begin{adjustbox}{width=\linewidth}
    \begin{tabular}{llcccc}
    \toprule
        Molecule & Metric & TorchMDNet & Joint & Pretrained Model & Finetuned Model \\ 
        \midrule
        Aspirin  & Forces &  10.9 & & & \\
                & Stability & & & & \\
                & h(r) & & & & \\
        Benzene & Forces &  8.4 & & & \\
                & Stability & & & & \\
                & h(r) & & & & \\
        Ethanol & Forces &  4.7 & & & \\
                & Stability & & & & \\
                & h(r) & & & & \\
        Malondialdehyde & Forces &  7.3 & & & \\
                & Stability & & & & \\
                & h(r) & & & & \\
        Naphthalene & Forces &  2.6 & & & \\
                & Stability & & & & \\
                & h(r) & & & & \\
        Salicylic Acid & Forces &  5.6 & & & \\
                & Stability & & & & \\
                & h(r) & & & & \\
        Toluene & Forces &  2.9 & & & \\
                & Stability & & & & \\
                & h(r) & & & & \\
        Toluene & Forces &  4.1 & & & \\
                & Stability & & & & \\
                & h(r) & & & & \\
        Average & Forces 6.0 & & & &
    \end{tabular}
    \end{adjustbox}
    \caption{}
    \label{tab:my_label}
\end{table}

==> exp/optim.tex <==
\section{Geometry Optimization}

==> tables/polymer_table.tex <==
\begin{tabular}{lllll}
\hline
Index         & Type                         & \# Atoms & Monomer                                                            & Polymer                                                            \\ \hline
\textbf{CK1}  & cyclopropane                 & 9       & \includegraphics[width=\molwidth]{pics/molecules/49-monomer.png}   & \includegraphics[width=\molwidth]{pics/molecules/49-polymer.png}   \\
\textbf{CK2}  & cyclobutane                  & 12       & \includegraphics[width=\molwidth]{pics/molecules/51-monomer.png}   & \includegraphics[width=\molwidth]{pics/molecules/51-polymer.png}   \\
\textbf{CK3}  & cyclopentane                 & 15      & \includegraphics[width=\molwidth]{pics/molecules/53-monomer.png}   & \includegraphics[width=\molwidth]{pics/molecules/53-polymer.png}   \\
\textbf{CK4}  & cyclohexane                  & 18       & \includegraphics[width=\molwidth]{pics/molecules/993-monomer.png}  & \includegraphics[width=\molwidth]{pics/molecules/993-polymer.png}  \\
\textbf{CK5}  & cycloheptane                 & 21       & \includegraphics[width=\molwidth]{pics/molecules/994-monomer.png}  & \includegraphics[width=\molwidth]{pics/molecules/994-polymer.png}  \\
\textbf{CK6}  & cycloctane                   & 24      & \includegraphics[width=\molwidth]{pics/molecules/995-monomer.png}  & \includegraphics[width=\molwidth]{pics/molecules/995-polymer.png}  \\ \hline
\textbf{ETH}  & ethylene oxide               & 7       & \includegraphics[width=\molwidth]{pics/molecules/50-monomer.png}   & \includegraphics[width=\molwidth]{pics/molecules/50-polymer.png}   \\ \hline
\textbf{LAC1} & \(\gamma\)-butyrolactone              & 9       & \includegraphics[width=\molwidth]{pics/molecules/52-monomer.png}   & \includegraphics[width=\molwidth]{pics/molecules/52-polymer.png}   \\
\textbf{LAC2} & \(\gamma\)-butyrolactone              & 12       & \includegraphics[width=\molwidth]{pics/molecules/7-monomer.png}    & \includegraphics[width=\molwidth]{pics/molecules/7-polymer.png}    \\
\textbf{LAC3} & 1,4-dioxan-2-one             & 13      & \includegraphics[width=\molwidth]{pics/molecules/15-monomer.png}   & \includegraphics[width=\molwidth]{pics/molecules/15-polymer.png}   \\
\textbf{LAC4} & \(\delta\)-valerolactone              & 15      & \includegraphics[width=\molwidth]{pics/molecules/17-monomer.png}   & \includegraphics[width=\molwidth]{pics/molecules/17-polymer.png}   \\
\textbf{LAC5} & 3-methyl-1,4-dioxan-2-one    & 16      & \includegraphics[width=\molwidth]{pics/molecules/1-monomer.png}    & \includegraphics[width=\molwidth]{pics/molecules/1-polymer.png}    \\
\textbf{LAC6} & \(\beta\)-methyl-\(\delta\)-valerolactone     & 18      & \includegraphics[width=\molwidth]{pics/molecules/5-monomer.png}    & \includegraphics[width=\molwidth]{pics/molecules/5-polymer.png}    \\
\textbf{LAC7} & \(\delta\)-caprolactone               & 18      & \includegraphics[width=\molwidth]{pics/molecules/9-monomer.png}    & \includegraphics[width=\molwidth]{pics/molecules/9-polymer.png}    \\
\textbf{LAC8} & \(\delta\)-decalactone                & 30      & \includegraphics[width=\molwidth]{pics/molecules/11-monomer.png}   & \includegraphics[width=\molwidth]{pics/molecules/11-polymer.png}   \\
\textbf{LAC9} & (-)-Menthide                 & 30      & \includegraphics[width=\molwidth]{pics/molecules/3-monomer.png}    & \includegraphics[width=\molwidth]{pics/molecules/3-polymer.png}    \\ \hline
\textbf{OTH1} & n-alkane sub \(\delta\)-valerolactone & 18      & \includegraphics[width=\molwidth]{pics/molecules/1050-monomer.png} & \includegraphics[width=\molwidth]{pics/molecules/1050-polymer.png} \\
\textbf{OTH2} & \(\alpha\)-Methylene-\(\gamma\)-butyrolactone  & 13      & \includegraphics[width=\molwidth]{pics/molecules/1060-monomer.png} & \includegraphics[width=\molwidth]{pics/molecules/1060-polymer.png} \\
\textbf{OTH3} & n-alkane sub \(\delta\)-valerolactone & 21      & \includegraphics[width=\molwidth]{pics/molecules/1052-monomer.png} & \includegraphics[width=\molwidth]{pics/molecules/1052-polymer.png} \\
\textbf{OTH4} & n-alkane sub \(\delta\)-valerolactone & 24      & \includegraphics[width=\molwidth]{pics/molecules/1053-monomer.png} & \includegraphics[width=\molwidth]{pics/molecules/1053-polymer.png} \\
\textbf{OTH5} & n-butyl \(\delta\)-valerolactone      & 27      & \includegraphics[width=\molwidth]{pics/molecules/1054-monomer.png} & \includegraphics[width=\molwidth]{pics/molecules/1054-polymer.png} \\
\textbf{OTH6} & n-alkane sub \(\delta\)-valerolactone & 30      & \includegraphics[width=\molwidth]{pics/molecules/1055-monomer.png} & \includegraphics[width=\molwidth]{pics/molecules/1055-polymer.png} \\
\textbf{OTH7} & n-alkane sub \(\delta\)-valerolactone & 33      & \includegraphics[width=\molwidth]{pics/molecules/1056-monomer.png} & \includegraphics[width=\molwidth]{pics/molecules/1056-polymer.png} \\
\textbf{OTH8} & n-alkane sub \(\delta\)-valerolactone & 42      & \includegraphics[width=\molwidth]{pics/molecules/1058-monomer.png} & \includegraphics[width=\molwidth]{pics/molecules/1058-polymer.png} \\ \hline
\end{tabular}

